Adversarial Text Generation via Feature-Mover's Distance

Generative adversarial networks (GANs) have achieved significant success in generating real-valued data. However, the discrete nature of text hinders the application of GAN to text-generation tasks. Instead of using the standard GAN objective, we propose to improve text-generation GAN via a novel approach inspired by optimal transport. Specifically, we consider matching the latent feature distributions of real and synthetic sentences using a novel metric, termed the feature-mover's distance (FMD). This formulation leads to a highly discriminative critic and easy-to-optimize objective, overcoming the mode-collapsing and brittle-training problems in existing methods. Extensive experiments are conducted on a variety of tasks to evaluate the proposed model empirically, including unconditional text generation, style transfer from non-parallel text, and unsupervised cipher cracking. The proposed model yields superior performance, demonstrating wide applicability and effectiveness.

==> result/human_yelp.tex <==
\begin{table}[h]
	\centering
	\small
	\def\arraystretch{1.0}
	\begin{tabular}{c|ccc}
		\toprule[1.2pt]
		% content: content preservation
		Model & Sentiment & Content &  Fluency \\
		\hline
		Controllable\cite{hu2017toward}    & 3.6 & \textbf{4.6} & 4.2   \\
		CAE \cite{shen2017style}       & 3.2 & 4.1 & 3.7  \\
		Ours         & \textbf{4.1} & 4.5 & \textbf{4.4} \\
		\bottomrule[1.2pt]
	\end{tabular}
	\vspace{2mm}
	\caption{Human evaluation for the quality of sentiment transferred sentences. }
	\label{tab:human_transfer}
	\vspace{-6mm}
\end{table}

==> result/table.tex <==
\begin{table}[H]%{r}{0.45\textwidth} 
\centering 
\begin{adjustbox}{scale=0.9,tabular=l | c | c | c | c | c | c | c | 
c,center} 
{Method}&MLE & SeqGAN & RankGAN & GSGAN & LeakGAN & VAE & textGAN & 
FMGAN\\ 
\hline\hline 
BLEU-2 & 0.820 & 0.820 & 0.852 & 0.810 & 0.922 & 0.926 & 0.910 &\\ 
BLEU-3 & 0.607 & 0.604 & 0.637 & 0.566 & 0.797 & 0.774 & 0.728 &\\ 
BLEU-4 & 0.389 & 0.361 & 0.389 & 0.335 & 0.602 & 0.552 & 0.484 &\\ 
BLEU-5 & 0.248 & 0.211 & 0.248 & 0.197 & 0.416 & 0.362 & 0.306 &\\ 
\end{adjustbox} 
\caption{ 
BLEU scores on COCO Image Captions. 
} 
\label{tab:COCOun} 
\vspace{-0.8cm} 
\end{table} 
\begin{table}[H]%{r}{0.45\textwidth} 
\centering 
\begin{adjustbox}{scale=0.9,tabular=l | c | c | c | c | c | c | c | 
c,center} 
{Method} & MLE & SeqGAN & RankGAN & GSGAN & LeakGAN & VAE & textGAN & 
FMGAN\\ 
\hline\hline 
BLEU-2 & 0.754 & 0.807 & 0.822 & 0.785 & 0.912 & 0.830 & 0.806 
&\textbf{0.746}\\ 
BLEU-3 & 0.511 & 0.577 & 0.592 & 0.522 & 0.825 & 0.597 & 0.548 
&\textbf{0.511}\\ 
BLEU-4 & 0.232 & 0.278 & 0.288 & 0.230 & 0.689 & 0.284 & 0.217 
&\textbf{0.319}\\ 
\end{adjustbox} 
\caption{ 
Self-BLEU scores on COCO Image Captions. 
} 
\label{tab:COCOunself} 
\end{table} 

\begin{table}[H]%{r}{0.45\textwidth} 
\centering 
\begin{adjustbox}{scale=0.9,tabular=l | c | c | c | c | c | c | c | 
c,center} 
{Method} & MLE & SeqGAN & RankGAN & GSGAN & LeakGAN & VAE & textGAN & 
AVAE\\ 
\hline\hline 
BLEU-2 & & 0.630 & 0.774 & 0.723 & 0.920 & 0.901 & 0.777 & 0.911\\ 
BLEU-3 & & 0.354 & 0.484 & 0.440 & 0.725 & 0.740 & 0.529 & 0.707\\ 
BLEU-4 & & 0.164 & 0.249 & 0.210 & 0.502 & 0.558 & 0.305 & 0.472\\ 
BLEU-5 & & 0.087 & 0.131 & 0.107 & 0.321 & 0.304 & 0.161 & 0.289\\ 
\end{adjustbox} 
\caption{ 
BLEU scores on EMNLP2017 WMT 
} 
\label{tab:wmt} 
\end{table} 
\vspace{-0.8cm} 
\begin{table}[H]%{r}{0.45\textwidth} 
\centering 
\begin{adjustbox}{scale=0.9,tabular=l | c | c | c | c | c | c | c| 
c,center} 
{Method} & MLE & SeqGAN & RankGAN & GSGAN & LeakGAN & VAE & textGAN & 
AVAE\\ 
\hline\hline 
BLEU-2 & & 0.728 & 0.672 & 0.807 & 0.857 & 0.917 & 0.806 & 0.798\\ 
BLEU-3 & & 0.411 & 0.346 & 0.680 & 0.696 & 0.815 & 0.662 & 0.563\\ 
BLEU-4 & & 0.139 & 0.119 & 0.450 & 0.553 & 0.676 & 0.448 & 0.331\\ 
\end{adjustbox} 
\caption{ 
self-BLEU scores on EMNLP2017 WMT. 
} 
\label{tab:wmtun} 
\end{table}

==> result/table_yelp.tex <==
\begin{table}[h]
  \centering
      \caption{Sentiment transfer accuracy on Yelp.}
      \footnotesize
    %   \begin{minipage}{1.\linewidth}
      \begin{tabular}{l|cccc}
        \toprule[1.2pt]
        {Method}& Controllable text~\cite{hu2017toward} & CAE~\cite{shen2017style} & BST~\cite{prabhumoye2018style} & Our model\\ 
        \hline
        Accuracy(\%) & 84.5 &  80.6 & 87.22 & \textbf{89.8}\\ 
        \bottomrule[1.2pt]
      \end{tabular}
      \vspace{-8mm}
      \label{table:yelp}
    %   \end{minipage}
%       \medskip
%       \begin{minipage}{0.5\linewidth}
%       \begin{tabular}{c|ccc}
% 		\toprule[1.2pt]
% 		% content: content preservation
% 		Model & Sentiment & Content &  Fluency \\
% 		\hline
% 		Controllable text \cite{hu2017toward}    & 3.6 & \textbf{4.6} & 4.2   \\
% 		Cross-aligned AE \cite{shen2017style}       & 3.2 & 4.1 & 3.7  \\
% 		Ours         & \textbf{4.1} & 4.5 & \textbf{4.4} \\
% 		\bottomrule[1.2pt]
% 	\end{tabular}
% 	\end{minipage}
\end{table}

==> result/temp.tex <==
\begin{minipage}[h]{0.5\linewidth}
% \begin{figure}[ht!]
  %\centering
%   \vspace{-27mm}
\resizebox{1.\linewidth}{!}{
\def\arraystretch{1.2}
\begin{tabular}{l|l}
			\toprule[1.2pt]	
			\textbf{Ground Truth}:&one of the best gourmet store shopping experiences i have ever had .  \\
			\hline
			\textbf{controllable }: &one of the best gourmet store shopping experiences i have ever had . \\
			\textbf{CAE}: &one of the worst staff i would ever ever ever had ever had . \\
			\textbf{Ours}:&one of the worst indian shopping store experiences i have ever had .\\
			\hline
			\hline
			\textbf{Ground Truth}:&staff behind the deli counter were super nice and efficient !\\
			\hline
			\textbf{Controllable}: &staff behind the deli counter were super rude and efficient !\\
			\textbf{CAE}: &the staff were the front desk and were extremely rude airport ! \\
		    \textbf{Ours}:&staff behind the deli counter were super nice and inefficient !\\
		    \bottomrule[1.2pt]
		\end{tabular}
		}
		\captionof{table}{\footnotesize xxxxxx.}\label{tab:xx}
\end{minipage}
\hspace{1mm}
\begin{minipage}[h]{.5\linewidth}

	%\vspace{-27mm}
	\resizebox{1.\linewidth}{!}{
	\def\arraystretch{1.2}
	\begin{tabular}{c|l}
			\toprule[1.2pt]	
			\textbf{LeakGAN}:&" i think we pride destroy racist export system and even\\ &potential links to russia , " and to ensure that the interests " of the\\ &government has been taken from the single market .   \\
			 &one of the best gourmet store shopping experiences i have ever had . \\
			 &one of the worst staff i would ever ever ever had ever had . \\
			&one of the worst indian shopping store experiences i have ever had .\\
			\hline
			\textbf{Ours}:&staff behind the deli counter were super nice and efficient !\\
			 &staff behind the deli counter were super rude and efficient !\\
			 &the staff were the front desk and were extremely rude airport ! \\
		     &staff behind the deli counter were super nice and inefficient !\\
		    \bottomrule[1.2pt]
		\end{tabular}
	}
	\captionof{table}{\footnotesize xxxxxx.}\label{tab:cer}
	% \vspace{-2mm}
% \end{table}
\end{minipage}


==> result/yelp2.tex <==
\begin{wrapfigure}[12]{R}{0.45\textwidth}
\begin{minipage}{0.45\textwidth}
\begin{table}[H]
  \centering
      \caption{Sentiment transfer accuracy on Yelp.}\label{table:yelp}
      \footnotesize
    %   \begin{minipage}{1.\linewidth}
      \begin{tabular}{l|cccc}
        \toprule[1.2pt]
        {Method}& Accuracy(\%) & Sentiment & Content & Fluency\\ 
        \hline
        Controllable~\cite{hu2017toward} & 84.5 & 3.6 & \textbf{4.6} & 4.2\\ 
        CAE~\cite{shen2017style} & 80.6 & 3.2 & 4.1 & 3.7 \\
        BST~\cite{prabhumoye2018style}   & 87.22 & - & - & - \\
        Our model    & \textbf{89.8} & 4.1 & 4.5 & \textbf{4.4} \\
        \bottomrule[1.2pt]
      \end{tabular}
      

\end{table}
\end{minipage}
\end{wrapfigure}

==> statistics.tex <==
\begin{table}
	\centering
	\def\arraystretch{1.2}
	\begin{tabular}{cccccc}
		\hline
		Dataset & Train &Test  &  Vocabulary & average \#w\\
		\hline
		CUB    & 10,0000  & 10,000  & 4,391 & \\
		MS COCO         & 120,000 & 10,000 & 27,842 & \\
		EMNLP2017 WMT         & 278,686 & 10,000 & 5,728 & \\
		\hline
	\end{tabular}
	\vspace{2mm}
	\caption{Data statistics}
	\label{tab:summary}
	\vspace{-6mm}
\end{table}
